Behavior Matters: An Alternative Perspective on Promoting Responsible Data Science

Data science pipelines inform and influence many daily decisions, from what we buy to who we work for and even where we live. When designed incorrectly, these pipelines can easily propagate social inequity and harm. Traditional solutions are technical in nature; e.g., mitigating biased algorithms. In this vision paper, we introduce a novel lens for promoting responsible data science using theories of behavior change that emphasize not only technical solutions but also the behavioral responsibility of practitioners. By integrating behavior change theories from cognitive psychology with data science workflow knowledge and ethics guidelines, we present a new perspective on responsible data science. We present example data science interventions in machine learning and visual data analysis, contextualized in behavior change theories that could be implemented to interrupt and redirect potentially suboptimal or negligent practices while reinforcing ethically conscious behaviors. We conclude with a call to action to our community to explore this new research area of behavior change interventions for responsible data science.

==> sections/2.ds_ameya.tex <==
\section{Responsible Behaviors in Data Science}
\label{sec:background_ds}

% \emily{somewhere in here state that it is outside the scope of this paper to put forth a definition of ethical/responsible data science -- instead, we review some common frameworks}

% \emily{move pipeline stuff to an appendix?}

% \emily{
%     \begin{enumerate}
%     \item Best Practices in Data Science (Technical Rigor) (evaluation metrics etc)
%     \item Frameworks for Ethical Rigor in Data Science
%     \item Practical Examples (applying these two sections)
%     \end{enumerate}
% }

% \ziwei{suggest we cut down (3) since section 2 is already 4 pages -- a bit too long considering we need to add in another 1/2 page for examples.}




%In this section, we consider constituent components of \textit{responsible behaviors in data science}. 


Analyzing data and drawing insights from them places significant power and consequently responsibility in the hands of the analyst since these insights can potentially affect policies on a large scale.
For example, when opaque models are used to make court rulings, it becomes impossible to understand why a decision was made or how biased inputs such as insufficient training data influenced the outcome~\cite{barabas2018interventions, ajunwa2019platforms}. Having realized this responsibility, the data science community has called for more deliberation on the ethics of current data science pipelines. Ehsan \etal\cite{ehsan2023human} argued that actionable interventions are in demand to recognize both affordances and potential pitfalls of data science and AI. 
As the main contribution of this paper is behavior change interventions for responsible data science, it is outside the scope of this paper to put forth a comprehensive review of the literature on responsible data science; however, it is necessary to first contextualize what target behaviors may look like in responsible data science. 
We organize this section by first defining and characterizing data science behaviors along two dimensions -- \textit{Agent} and \textit{Desired Outcome} in ~\autoref{sec:outcomes_agents} (also shown in ~\autoref{fig:teaser}). %distinguishing between technical and human agents; and satisfactory and responsible data science outcomes in \autoref{sec:outcomes_agents}.
% We outline technically satisfactory data science that has traditionally been focused upon (\autoref{}) and envision what it means for data science to be behaviorally responsible(\autoref{}). 
We also connect the examples in~\autoref{fig:examples} with this characterization alongside.
% We outline satisfactory data science that has traditionally focused on the technical agent in~\autoref{sec:technical_satisfactory} and envision what it means for data science to be behaviorally responsible in~\autoref{sec:behaviorally_responsible}.
%\emily{I'm leaning towards removing the final subsection on examples, and instead just incorporating those examples into the respective sections...}



% This dual classification aligns responsible data science along technical and ethical axes, creating a comprehensive framework that marries methodological rigor with ethical contemplation. Such an approach fosters conscientious and impactful data science practices, while emphasizing the harmonious relationship between precise technical execution and principled ethical conduct.
%\emily{I would suggest to move this paragraph to be the first in the section -- then transition to say something like "We categorize data science practices along two dimensions: x and y, to describe the differences in approach to responsible data science and data science best practices." Then maybe a bolded header before 2.1 that says like "Outcomes and Agents" and that's where we include the definition of these categories? Although... introducing teaser here in this section makes it feel incomplete if we talk about  rows 1/2 but not the dimension covered by left/right columns}\ziwei{addressed this problem by moving the first paragraph of this section to section 1.}


% \ameya{Need revision as per Yuichi's 2x2 table to address the definitions of Satisfactory and Responsible behaviors, and Technical and Ethical rigor. Also mention that we only discuss behavior change examples for purely ethical rigor (bottom right box in~\autoref{fig:teaser}) for DS domain examples} \ziwei{addressed on the above two paragraphs}

% \ameya{As we go from top left to bottom right, does the focus on motivation increase compared to opportunity and capability, to achieve behavior change? Because of the very nature of behaviorally responsible domain? Or we can say that as per COM-B, both capability and opportunity in turn also increase motivation, so the focus falls on motivation eventually. Need to avoid making sweeping statements or pitching something new on behavior studies.}

% In this section, we (i) detail technically responsible best practices in data science, (ii) identify ethical behaviors in data science.




\subsection{Characterizing Agents and Outcomes of Responsible Data Science}
\label{sec:outcomes_agents}
% Herein, we focus on reviewing some common frameworks of responsible data science, including concepts of technical and ethical rigor.
%In our investigation of responsible behaviors in the field of data science, we delineate responsible data science can be promoted mainly via two important parts: \textbf{technically satisfactory behaviors} and \textbf{behaviorally responsible behaviors}. The division of responsible data science into these two components establishes a framework that navigates the complex terrain of data-driven research with clarity. 
%In the context of behavior change interventions, we can consider technical and behavioral responsible behaviors as two categories of target behavior we would like for interventions to influence. 
To distinguish between prior work in data science and our new perspective on behavior change, we find it useful to characterize the space of responsible data science into two dimensions (as shown in ~\autoref{fig:teaser}): \textit{agents} and \textit{desired outcomes}. 
The first dimension, agent, can be \textit{technical} or \textit{behavioral}. 
Technical agents represent systems or techniques used in data science that have the potential to influence the rigor of data science practice through technical indicators, algorithms, systems, and toolkits that are incorporated in the data science project. Behavioral agents, on the other hand, represent humans performing actions that affect the rigor of data science practice.
%, such as knowing when/why to apply certain techniques or empirically examining the downstream consequences of a deployed model.

The second dimension, desired outcome, indicates the extent of attention to care and responsibility the data science practitioners pay in the data science practice. 
We categorize desired outcomes loosely as either \textit{satisfactory} or \textit{responsible}. 
%Satisfactory outcomes encompass technically satisfactory best practices that practitioners follow such as ensuring sufficient model accuracy. 
Satisfactory outcomes means following the established best practices, while responsible outcomes go above or beyond the current norms of technically best practices to minimize harm, and actively benefit society. 

We note that \textit{technically satisfactory} best practices (\autoref{fig:teaser}A, green cell) have traditionally been the focus of data science practitioners. 
It involves among many examples, using tools which help us quantitatively evaluate and optimize the model. % thoughtfully selecting data and implementation methodologies. \ameya{thoughtfully selecting data and implementation is behaviorally satisfactory}
In this paper, we highlight the complementary importance of \textit{behaviorally responsible} practices (\autoref{fig:teaser}D, red cell) in promoting responsible data science. 
Behavioral responsibility underscores the broader societal implications that are interwoven into data science. Acknowledging the far-reaching effects that analyses can have on policies and individuals, this facet prompts data scientists to examine potential risk and harm, address privacy concerns, ensure fairness, and consider broader social impacts. 

\begin{comment}
In the smoking cessation example, we can characterize desired outcomes as satisfactory (e.g., that an individual stops smoking to improve their own health) and responsible (e.g., that an individual stops smoking to improve the health of others around them by not contributing to second-hand smoke). The agent of that outcome can be technical in nature (e.g., creating less harmful cigarettes) or human in nature (e.g., relying on behaviors and habits). 
In the context of carbon footprint management, desired outcomes can be satisfactory (e.g., that an individual makes more sustainable personal choices) and responsible (e.g., that an individual advocates that corporations accept responsibility for carbon footprint emissions). The agent can be technical in nature (e.g., creating more sustainable packaging) or human in nature (e.g., choosing to take public transit rather than drive).

In the data science domain, the machine learning example may have satisfactory desired outcomes such as a data scientist ensuring a sufficiently accurate model, and responsible desired outcomes such as a data scientist investigating the fairness of the model and applying appropriate corrections. Technical agents in this case could be, for example, systems that alert users to inadequate generalizability, while human agents could include data scientists engaging in the collection of new, unbiased datasets using responsible methodologies.

In the visual data analysis context, satisfactory desired outcomes could include the use of visualizations that show accurate representations of data, while responsible outcomes might likewise involve use of visualizations that show accurate representations of data, but with emphasis on representations that viewers can easily comprehend. 
Technical agents could include choosing proper techniques to visualize the data, while human agents could involve engaging in user-centered design practices.
\end{comment}

% \emily{TODO: reframe throughout the paper -- responsible v. ethical}



% \emily{Todo: for the new teaser, can cite some of my work on bias where we look at behavioral indicators of bias rather than outcomes of decisions}



\subsection{Technically Satisfactory Behaviors for Responsible Data Science}
% \ziwei{todo on monday: transit into technical part, cite bias in ml , and gt xai paper here. say the checklist can help data scientists to be more responsible on tech side}

\label{sec:technical_satisfactory}



In the broader landscape of data science, the intricacies and nuances of every step of the data science pipeline demands meticulous attention to technical details. Every step presents opportunities for decisions that can significantly influence outcomes. To guide data scientists in this endeavor, a systematic approach is indispensable. A notable resource in this regard is the comprehensive survey conducted by Mehrabi~\etal\cite{mehrabi2021survey}. We refer to it as an insightful guidepost of potential sources of bias we should be mindful of within data science practices. In this subsection, we delve into the specifics of technically satisfactory behavior, elucidating the key aspects that demand vigilance and adherence to best practices. Due to the comprehensiveness of \cite{mehrabi2021survey}, we derive a technical checklist for technically satisfactory behaviors based on the potential technical bias in data science practices proposed by Mehrabi~\etal, which we hope to promote for data science: 


\begin{itemize}
    
    
    \item \textbf{Choosing appropriate statistical tests:}
    After a research hypothesis is formulated, a suitable statistical test must be used to verify it. However, since domain experts may not be well-versed with statistics, the selection of appropriate statistical tests (\eg one-way or two-way ANOVA) and parameters like significance level must be carefully considered. Binnig~\etal~\cite{binnig2017toward} provide this kind of statistical guidance to the analyst in their QUDE system. Jun~\etal~\cite{tea} compile high-level specifications into a constraint satisfaction problem that determines the set of valid statistical tests. 
    %Another work of Jun~\etal~\cite{jun2022tisane} proposed a system that guides users to author generalized linear models and generalized linear models with mixed-effects
    %\emily{Can also mention Eunice Jun's work on Tea and Tisane for selecting statistical tasts}\ziwei{addressed}
    \item \textbf{Choosing proper data science models:} The choice of model can significantly impact the quality of results and the ability to make meaningful predictions or decisions~\cite{ding2018model,khaledian2020selecting}. It begins with a deep understanding of the problem at hand and the characteristics of the data. Depending on the nature of the data, different models may be more appropriate, whether it is a decision tree for interpretability, a deep neural network for complex patterns, or a linear regression model for simple relationships. Moreover, model selection should consider factors such as scalability, computational resources, and interpretability, depending on project requirements. Regularization techniques and hyperparameter tuning further refine model performance. In some cases, ensemble methods or domain-specific models may be preferred. The process of choosing the right model should be driven by a comprehensive analysis of the problem, data, and project objectives, ensuring that the selected model is not only technically sound but also best suited to deliver actionable insights or predictions.
    
    \item \textbf{Choosing suitable evaluation metrics:} Choosing appropriate evaluation metrics is a pivotal aspect of ensuring a technically sound data science project. It is crucial to align the choice of evaluation metrics with the project's specific objectives \cite{zhou2021evaluating}. Depending on whether the task involves classification, regression, or clustering, different metrics such as accuracy, precision, recall, F1-score, or Mean Absolute Error (MAE) should be carefully considered. Additionally, the presence of imbalanced data or unique business considerations may warrant the use of specialized metrics. Domain knowledge and collaboration with subject matter experts can further guide the selection of metrics that best reflect the real-world impact of the data science solution. 
    
    
    \item \textbf{Interpreting correlations correctly:} The correct interpretation of data correlations is crucial in data science to avoid incorrect conclusions of causation from an association\cite{dhar2013data}. Correlation measures the relationship between variables but does not establish cause and effect. Misinterpreting correlation as causation can lead to flawed decisions and strategies. Data scientists should exercise caution, communicate the limitations of correlation, and conduct further research to determine true causal relationships accurately. Understanding this distinction enables responsible decision-making and effective strategies based on reliable evidence. \emily{this one doesn't seem to "fit" as naturally under technically satisfactory... as it is based on human interpretation rather than system. don't move it immediately, but let's discuss. I'm curious what others think?}\ziwei{agree, i vote for moving it to the next subsection, what others think?}
    
    \item \textbf{Visualizing or communicating results:}
    Correll~\cite{correll2019ethical} calls for communicating the results of data analysis sessions with consideration for the data context and uncertainties, especially when using the medium of visualizations, which can abstract or trivialize the context provided by the data. One example is the proposed use of fuzzy gradient plots instead of well-defined bar charts to better convey the uncertainty in the data~\cite{correll2014error} .
    
    
    % \emily{any notable points from these checklists that we may want to call attention to?}
    
\end{itemize}


% What are the prerequisites to create a framework to intervene to elicit responsible behaviour during data analysis?



\subsection{Behaviorally Responsible Practices in Data Science}
%\ziwei{please note that this subsection has many wording of "ethical/ethics" I did not change it to responsible as I think they are mainly used for literature purposes, and it is ok to use the wording ethical here. Please comment if you have other opinions.}

\label{sec:behaviorally_responsible}


There are several approaches for considering behavioral responsibility of data scientists, such as the approach by Aragon \etal\cite{aragon2022human} who proposed ethical principles in Human-Centered Data Science, Heise \etal\cite{heise2019internet} who curated primary ethical norms in computational research, and Zegura \etal\cite{zegura2018care} who called for taking care and social good into consideration when conducting data science practices. Among the prominent literature we reviewed, we primarily draw upon the insights from \textit{Human-Centered Data Science}\cite{aragon2022human} and the concept of \textit{Care and the practice of data science for social good}\cite{zegura2018care}. 
These two approaches offer complementary perspectives because they emphasize the importance of responsible motivation when conducting data science practices and characterize actionable solutions to facilitate ethical practices in data science. 
While \textit{Human-Centered Data Science} primarily emphasizes high-level principles and guidelines for practicing data science with care and rigor, \textit{Care and the practice of data science for social good} delves into the details of responsible practices at each stage of the data science pipeline, such as problem understanding and data preparation. 
We next describe these two approaches in greater detail. 


First, \textit{Human-Centered Data Science}\cite{aragon2022human} provides a foundational resource that facilitates a systematic approach to contemplating behaviorally responsible practices within the realm of data science. Within its pages, the book offers a comprehensive set of ethical guidelines that encourage a nuanced consideration of data science projects, \eg ethics on defining the data science problem and ethical principles of training, validating, and testing data science models. The authors emphasize the key characteristic of responsible data science: ``Our goal here is to make you aware that thinking critically and caring about your process and how it affects your results, as well as the people whose behavior is represented in your dataset, is needed every step of the way'' \cite{aragon2022human}.
% actively thinking through the decisions and practices throughout the process, and being aware and caring about how decisions made in data science contexts could affect results. \emily{can you replace this point with a quote?}
% This approach takes into account a diverse array of potential scenarios and contexts, in contrast to an oversimplified checklist or a rigid rule-based ethical framework. \emily{this sentence seems odd- lkke checklists and frameworks do not cover multiple scenarios. can you rephrase this? i suspect these points are orthogonal and the distinction between these approaches should be articulated differently}
The applicability of these ethical guidelines is notably well-suited to a wide range of situations where humans are, or ought to be, involved, such as loan approval and criminal recidivism predictions. 

% Care and the practice of data science for social good


Second, the authors of \textit{Care and the practice of data science for social good}\cite{zegura2018care} argued responsible practices are informed by a thoughtful examination of  \textit{how} research is done and in what \textit{context} it is done. It argues responsible data science relies on an ethics approach rooted in practicality: ethics involves not only adhering to formal rules or their definitions but also observing actual behaviors. Ethics shouldn't be treated as a goal to optimize or ``manipulate.'' 
%\emily{emphasize again here why these two approaches are complementary/similar / different/valuable}\ziwei{made an attempt to address it, please see the following text}
%While these two approaches differ in their focus, we have discovered that they complement each other. 



We assert that ethics requires a continuous process of reflection—considering potential risks, benefits, and possible harms. Yet, ethics goes beyond reflection; being thoughtful alone does not necessarily prevent harm. Data scientists might need to collaborate with relevant parties, especially those whose data is utilized in analyses. At each stage of the data science pipeline, new ethical questions and challenges can emerge, demanding attention and resolution. The imperative to embrace responsible behaviors in data science emerges from the recognition that a singular, fixed, and standardized checklist are often insufficient across diverse scenarios encountered in the field \cite{aragon2022human}. Instead, behaviorally responsible data science practices demand that practitioners proactively apply thorough attention and resolution to dynamically consider the nature of the specific data science problem and context. Thus, a reflexive and adaptable stance is essential, acknowledging that the ethical considerations surrounding each data science project are nuanced and distinct. 
This diversity underscores the pivotal role of "\textbf{Care Ethics}", a key concept to both \textit{Human-Centered Data Science} \cite{aragon2022human} and the concept of \textit{Care and the practice of data science for social good} \cite{zegura2018care} as a foundational principle guiding behaviorally responsible data science. \emily{need to cite something on care ethics}
%We have observed that Human-Centered Data Science offers a valuable high-level mindset for practitioners to follow when designing data science solutions. On the other hand, caring data science for social good provides detailed concrete examples of the behaviors that practitioners should be mindful of at each step of the data science pipeline.

%\emily{introducing human-centered data science as a primary framework seems contradicted by now introducing caring ethics as the primary framework... are both of these contributing something unique? can you justify them both and describe why both are complementary and relevant?}
%\emily{we also say we can't have a checklist, then introduce a checklist. This is contradictory}\ziwei{made an attempt to address the comments, but need eye on it to see if the current flow works well}\ziwei{before providing the list, i mentioned: "we review common data science practices reported in the literature and identify exemplary particularly promising activities that align with caring ethics". Would this be enough to cancel the potential contradiction of checklist thing? IMO we are not providing a checklist but instead, exemplify a subset of actionable responsible behaviors that we could promote.}
%\emily{I like the argument that a checklist approach is not sufficient, that we need a flexible and adaptable stance -- can we be a little more concise in getting to that point perhaps?} \leilani{agreed!}\ziwei{Attempted to address it}

Care Ethics encourages data scientists to approach their work with a deep sense of empathy and conscientiousness. It serves as a catalyst for thoughtful consideration of the potential risks and harms associated with decisions and actions taken during the data science process. By embracing this principle, data scientists adopt a mindset that prioritizes minimizing harm and maximizing benefit to all stakeholders involved. This approach prompts practitioners to reflect on how their choices would impact individuals, communities, and society at large. The notion of Care Ethics introduces a transformative shift in perspective. Encouraging data scientists to envisage their data science projects as endeavors involving their own family and loved ones cultivates a heightened sense of responsibility. This shift compels practitioners to go beyond technical and methodological considerations, delving into the profound societal and ethical implications of their work. Promoting Care Ethics not only enhances the behavioral responsibility of data science but also infuses the decision-making process with an intrinsic sense of accountability. %Inspired by the principle of caring ethics, 

Inspired by the principles contained within care ethics, we review some actionable activities that align with behaviorally responsible data science. 
These practices are not exhaustive and should not be viewed as a checklist -- instead, these serve only as inspirational examples to further ground the concept of behavioral responsibility in data science. %but consists of examples of responsible behaviors to further ground the concept.


%\emily{these only align with caring ethics, or they align with behaviorally reaponsible ds? also make sure the list has citations throighout for where these came from; add a statemwnt that says these are not exhaustive and should not be viewed as a checklist which we do not strive to promote as the best approach, but consists of examples of responsible behaviors to further ground the concept}\ziwei{addressed, updated the flow of the previous two sentences so it sticks with behavioral responsible data science instead of only caring ethics.}
%exemplify a list of behaviorally responsible behaviors we aim to promote for data science: \emily{wait, didn't you just make the point that we can't simplify it down to a list?}

% By promoting "caring ethics," data scientists are inspired to become proactive agents of positive change. This principle propels them to critically examine their decisions, anticipate potential challenges, and seek ways to mitigate any negative repercussions. In essence, "caring ethics" fosters a culture of ethical mindfulness that resonates across every stage of the data science pipeline. This paradigm shift, rooted in empathy and a dedication to the well-being of all, serves as a powerful catalyst for advancing the ethical dimensions of data science, driving toward a future where responsible and caring practices define the landscape of data-driven decision-making.




\begin{enumerate}

    \item \textbf{Comprehensive problem understanding\cite{zegura2018care}: } Understanding the data science problem in an unbiased way is fundamental to behavioral responsibility in data science. It starts with a clear recognition that preconceived notions or biases should not shape problem formulation. Data scientists must approach the problem with an open mind, free from personal or organizational biases that could skew the analysis or results \cite{van2016data}. It is essential to involve diverse perspectives and stakeholders to ensure a comprehensive understanding of the problem's nuances and potential impacts on different groups. Beyond that, attention should be paid to examining historical data, and considering the historical context of the problem as it could reveal biases or systemic inequalities that need to be addressed. This process also allows our partners to elaborate on what the community cares about and how the community envisions putting its care into practice through data.

    \item \textbf{Collecting unbiased data\cite{zegura2018care}:} Attention should be paid to unbalanced datasets, because imbalances can lead to biased models that perform poorly on minority classes. Data science practitioners may consider solving this issue by gathering more data for the minority classes, oversampling minority classes, or increasing the weight of the minority class to deal with the issue \cite{viloria2020unbalanced}.
    Systems like Trifacta~\cite{trifacta} enable dataset anomaly detection and quality assessment using quality rules such as data integrity constraints. Apart from that, consideration also needs to be given to data points which do not even exist in the collected dataset~\cite{gitelman2013raw}, which can potentially give us a biased starting point. 

    \item \textbf{Careful data preparation\cite{zegura2018care}: } Another pivotal step in the data science journey is data preparation, which holds immense significance for behaviorally responsibility in the field. The process of data preparation involves meticulously cleaning and wrangling datasets, ensuring that the data is accurate, complete, and free from bias \cite{brownlee2020data,van2016data}. Techniques such as handling missing values, outlier detection and treatment, and addressing data imbalances are crucial in creating a reliable foundation for subsequent analyses. In terms of caring data science, behaviorally responsible data preparation extends to the responsible handling of sensitive information, anonymizing data when necessary, and safeguarding privacy to uphold behaviorally responsible standards. Transformation techniques, such as feature engineering, enable the addition of meaningful attributes that contribute to a deeper understanding of the problem.
    
    \item \textbf{Identifying biased interactions with data\cite{aragon2022human}:}
    Identifying when bias may occur during analysis or interpretation, especially during interactive data analysis where the analyst may selectively look at certain data points while neglecting others (even though inadvertently)~\cite{kahneman2011thinking} is also a crucial step. Wall~\etal~\cite{wall2017warning} propose an approach of computing and visualizing bias in user interactions during visual analysis. Zgraggen~\etal~\cite{zgraggen2018investigating} propose confirmatory strategies to account for repeated testing or the multiple comparisons problem, to avoid \textit{p-hacking}, during exploratory visual analysis. 
    
    \item \textbf{Provenance tracking for accountability\cite{aragon2022human}:}
    It is easy to get side-tracked due to more interesting but illusory patterns in data, and enter into a rabbit-hole. To avoid such situations, it becomes necessary for the analysts to be aware of the individual steps during analysis as well as their high level approach. To facilitate this, visual analysis systems with provenance tracking have been created~\cite{callahan2006vistrails,feng2017hindsight,wood2019design} to help keep analysts grounded.
    
    \item \textbf{Streamlining pipelines with checklists\cite{aragon2022human}}: 
    At the commercial level where stakes are typically high, checklists have been created to draw developers' attention to the entire pipeline specifically in machine learning-based data science~\cite{jobin2019global, cramer2019translation, madaio2020co-designing}. Notable tasks within these checklists among many others, include ensuring fairness and privacy during data collection (\eg Is the population subject to inferences drawn from the collected data, correctly represented in the data? Do we have appropriate consent to gather the data?), transparency during analysis (\eg Can we reproduce the steps performed during this analysis?), and interpretability during inference (\eg Which factor was given more weight in a certain decision?).
\end{enumerate}

\begin{comment}
\subsection{Practical Examples}
Having discussed the different dimensions and corresponding required rigors for responsible data science behaviors, we now provide real-world examples. We also build parallels between the examples from the clinical and environmental sciences domains which have seen prior work from behavior change perspective, and the data science domain, as shown in~\autoref{fig:examples}. \autoref{sec:bc_psych} then describes the behavior change approach to be taken to induce the behavior change, and~\autoref{sec:interventions} provides example interventions for the same.

\subsubsection{Smoking Cessation}
Adam, a chain smoker is seeking help to get rid of his addiction. To give up his addiction, Adam first needs to identify when he feels the urge to smoke, so that he can take the necessary next steps accordingly. This calls for a desired \textit{satisfactory} behavior of being able to detect the tendency to relapse in the first place. Since this step may itself turn out to be difficult~\cite{paay2015understanding}, we focus on technical solutions to this problem. We thus need to design interventions focusing on \textit{technical} aspect owing to the desired \textit{satisfactory} behavior and the need to look at \textit{technical} agents.

\subsubsection{Carbon Footprint Management}
The city council of Bienville is rallying its residents to contribute towards making Bienville eco-friendly by changing their lifestyles. Unlike the previous example of smoking cessation, this example asks for a \textit{responsible} behavior from the citizens of Bienville. To move from \textit{technical responsibility} towards \textit{behavioral responsibility}, we will focus on the \textit{human} agent for this particular example.

\subsubsection{Machine Learning}
Moving to the data science domain, a machine learning startup in its initial phase of prototyping and gathering funding, is placing heavy emphasis on identifying which populations their models do and do not work on. However, for the hypothetical case where the startup works with a previously unused dataset, the data scientists are required to exhibit \textit{responsible} behavior. It is completely up to the \textit{human} agents in the form of the data scientists, to identify the caveats and publicise their idea accordingly.

\subsubsection{Visual Data Analysis}
A reputed journalism firm with a significant number of readers is creating data-driven stories in a wide variety of contexts. In the process of creating the required visualizations, they want to ensure that they are not designing visualizations which are far away from standard practices which can possibly result in misinterpretation or trivialization of the context~\cite{correll2019ethical}. This calls for a \textit{satisfactory} behavior on the part of the \textit{human} agent \ie the visualization designer.

With the last two examples in the data science domain, we demonstrate that responsible data science is not merely a theoretical concept but a tangible and vital approach in today's data-driven landscape. We thus drive our call-to-action towards focusing on the \textit{human} agent when working with data.


\end{comment}

% \subsubsection{A Healthcare Analytics Project}
% Bob, a data scientist working on a healthcare analytics project, exemplifies both technical and ethical responsibility throughout his work. In embracing technically responsible behaviors, Bob takes the time to comprehensively understand the healthcare problem he's addressing, engaging with healthcare professionals to define clear objectives that prioritize patient well-being. This aligns seamlessly with ethical responsibility by ensuring that the project's goals are grounded in ethical considerations. Bob collects unbiased data by collaborating with healthcare providers to assemble a diverse and representative dataset while proactively addressing potential biases tied to patient demographics. He upholds ethical principles by adhering to stringent data security protocols to safeguard patient confidentiality. Bob's commitment to data preparation involves meticulous cleaning and preprocessing, handling missing values and outliers to ensure the accuracy of his analyses. He further promotes technical responsibility by selecting appropriate healthcare-specific evaluation metrics, such as sensitivity and specificity, and interprets correlations correctly to guide informed decisions about patient care. Bob's transparent communication of results through easy-to-understand visualizations promotes responsible data science practices, allowing healthcare providers to make ethically sound decisions regarding patient treatment and care plans.

% \subsubsection{An Environmental Impact Assessment Project}
% Lily, a data scientist engaged in an environmental impact assessment for a manufacturing company, showcases her commitment to both ethical and technical responsibility throughout her project. She leads with ethical responsibility by considering the potential environmental and social consequences of her work, fostering a more comprehensive understanding of the problem's broader implications. In collecting unbiased data, Lily collaborates closely with environmental organizations, ensuring that her dataset accurately represents the affected communities. Her emphasis on transparency in data collection, including disclosure of data sources and potential conflicts of interest, underscores her ethical dedication. In data preparation, Lily anonymizes data to protect the privacy of individuals living near the manufacturing site and documents data sources and limitations to address potential biases related to data collection. Her choice of suitable evaluation metrics prioritizes environmental and societal well-being, emphasizing measures of pollution reduction and community impact. Lily's correct interpretation of correlations helps her understand the intricate relationships between manufacturing processes and environmental outcomes. Additionally, she streamlines her data science pipeline with checklists and provenance tracking, fostering accountability and transparency in her analyses. Lily's exemplary practices serve as a model for ethically and technically responsible data science, showcasing the importance of considering the broader societal and environmental implications of data-driven decisions.
\emily{todo: consolidate the examples provided in this section + 2.1 -- either remove the examples from the end of 2.1 and just mention them here, or move these examples up to 2.1}

==> sections/4.interventions.tex <==
\section{Interventions}
\label{sec:interventions}

% In this section, we envision possible interventions to facilitate positive behavior change in data science from both
% technical satisfactory and behavioral responsible aspects. We 

Given the responsible behaviors and theories of behavior change in the context of data science in the previous sections,
we now move on to envision some example behavior change interventions in data science. In this section, we refer back to the two data science contexts in \autoref{fig:examples} to discuss potential interventions for both the desired technically satisfactory and behaviorally responsible practices for the machine learning example in the third column, and visual data analysis example in the fourth column. We also provide additional examples of behavior change interventions in each domain context, demonstrating the generative power of the behavior change theories described in~\autoref{sec:bc_psych}.
% (1) highlight potential in-the-moment interventions for the machine learning example in the third column, (2) put forth a variety of potential interventions designed for the visual data analytics example in the fourth column. 
Note that this is not an exhaustive account of interventions for these two contexts but merely describes some possibilities, grounded in behavior change theory.
% (3) broaden the scope of our discussion to encompass a wider range of intervention design possibilities, extending beyond the examples that have thus far introduced.


\subsection{Interventions in a Machine Learning Workflow}

\leilani{I hate the term ``behaviorally responsible behavior''. It is redundant and makes us sound silly. I would prefer almost anything over it, actions, decisions, practices, etc. Please change.}
To achieve the behaviorally responsible practices of examining model decisions for any downstream consequences, we could educate data scientists about the possible ill-effects of their deployed ML models on the target groups. This intervention approach employs the Behavior Change Technique of shaping the knowledge of data scientists about the kind of power their models hold over the daily lives of people. The idea is that such training would change their attitude towards the kind of behavior they show when evaluating their models - the Mechanism of Action. Eventually this would affect the motivation (Factors affecting Behavior Change) of data scientists to change their workflows or decision processes to incorporate this crucial verification step of understanding the downstream consequences of their work.
\leilani{How would this be operationalized? This sounds a lot like a class which is out of scope. What is something a system could do?}

In terms of the reaching the desired technically satisfactory behavior of using multiple model accuracy metrics, we could train data scientists to make them aware of the numerous accuracy metrics for evaluating ML models, and the applicability of each metric in different use cases. Similar to the previous example, this intervention approach also employs the Behavior Change Technique of educating or training data scientists about the various evaluation metrics. Such an intervention would work by increasing the skills (Mechanism of Action) or the capability of the data scientist (Factors affecting Behavior Change) and induce a behavior change of using the appropriate metrics of model accuracy as per the demands of the use case.
\leilani{This is too high level, and again, sounds like a lecture in a class. How about the system generates metric recommendations with explanatory text regarding why it might be a good idea for a certain use case. Then, maybe we can mention potential future research is developing algorithms to detect appropriate contexts for each metric.}

\leilani{These examples basically seem to imply that digital interventions are useless and people should just teach each other? It sort of invalidates the paper?}
Such training sessions could be a part of the initial project setup, a mandatory training session for new joinees in the organization, or could be in-the-moment interventions when the data scientist moves from model training phase to model evaluation phase, or is about to deploy the model.

In addition to these two examples from~\autoref{fig:examples}, we can envision other helpful interventions throughout an ML workflow.
%Referring to the machine learning example in \autoref{fig:examples}, interventions could be designed to facilitate responsible practices throughout all phases of the data science pipeline. 
%\emily{I expected that the first part you would address is explicitly the intervention described in fig 2 (educate data scientists about potential bad impacts of model decisions on the target groups -- where in your pipeline can that happen? then if you want, you can add other examples (e.g., In addition to the example described in Fig. 2, we can envision other helpful interventions throughout the data science process. (...)}
At the beginning of an ML project for instance, the establishment of a clear project goal is of paramount importance. These goals could be based on technical indicators such as fairness metrics and/or evaluation approaches to achieve certain responsible outcomes in terms of downstream consequences. To that end, deploying a goal-setting prompt (Behavior Change Technique) while setting up the project, such as when creating the project notebook, can encourage the data scientist to form a concrete objective (\autoref{fig:intervention}). Such an intervention increases the capability (Factors affecting Behavior Change) of the data scientist to set up the pipeline effectively by giving them clarity about the goals. It also keeps them anchored to the end goal throughout the entire process through behavioral regulation (Mechanism of Action).
\leilani{this should probably focus on socially responsible goals to reinforce the point of the paper. If the goal is to produce technically satisfactory results, it weakens our argument.}

% \emily{may also want to be clear that the goal you are priming may be based on technical indicators like fairness metrics and/or other responsible outcomes that are the target goals}
With the goals established, it is crucial to consider the data preparation phase to check for issues such as missing values or labels. In this phase, interventions could take the form of prompts that remind data scientists to conduct these checks on data quality, completeness, or fairness. The prompts could manifest as tooltips providing guidance on how to handle missing data—for instance, suggesting techniques like replacing missing values with the dataset's average.  \leilani{this is a technically satisfactory solution. Is that on purpose?}

Within the feature engineering phase of the data science pipeline~\cite{}, 
%interventions serve to reinforce the importance of thorough consideration. Specifically, they
interventions can prompt data scientists to reevaluate whether there are any additional attributes that might prove valuable for the data science task (\autoref{fig:intervention}), or whether the selected features could potentially cause information leakage \emily{what do you mean by information leakage? like from a privacy perspective?} towards the data labels. 

During model deployment, interventions can take the form of pop-up reminders to encourage data scientists to explore different models and parameters for a more comprehensive comparison, aiding in the selection of the most suitable model for the data science task. 
\leilani{A more relevant trigger might be that if the system detects the user is close to deployment, it asks the whether users from marginalized groups were involved in the development process prior to deployment. In this way, it reminds the data scientist that everyone deserves to have their voices heard in terms of how these larger models/systems affect them.}

Upon the model evaluation phase, interventions can prompt data scientists to consider the broader problem context and its impact on the target sub-groups that are influenced by the model outcome. For example, a prompt may encourage reflection on whether the model draws inferences about populations that were underrepresented or excluded from the training dataset; or an automated model performance evaluation technique could issue alerts to data scientists when the model's performance or fairness metrics fall below a predefined threshold. 

In addition to interventions tailored for specific data science phases, general interventions that aim at enhancing data scientists' capabilities and knowledge could be applied in any phase of the data science pipeline \eg when faced with unfamiliar data cleaning or the training of new machine learning models. These facilitator \emily{facilitator is defined where?}interventions may involve the provision of quick-to-learn tips for immediate assistance or recommendations for technical tutorials and online courses to bridge the knowledge gaps. \leilani{Still seems too technical. I feel like I'm not seeing convincing behaviorally responsible actions.}

\emily{I was also expecting to see in this section that you talk through the behavior change technique, factors, and mechanisms of action for how this intervention would work}



\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figs/intervention.png}
    \caption{
    As an analyst starts analyzing a new dataset within a Jupyter notebook---here, US health survey data from the CDC and National Center for Health Statistics---we can monitor the user's notebook editing behavior to introduce interventions. For example, the creation of the notebook can be a good timing to deploy a goal-priming intervention to encourage the analyst to form concrete and testable hypotheses prior to exploration. Switching to a new phase of the data science pipeline---here, from data exploration to modeling---can be a good timing for introducing interventions, such as reminders to consider alternative data attributes. 
    }
    \label{fig:intervention}
\end{figure}

\subsection{Interventions Designed for Visual Data Analytics Example}
\emily{let's be sure we have illustrations for both 4.1 and 4.2, and make sure they cover the specific }
In the case of visual data analytics example in \autoref{fig:intervention}, where the goal is to communicate and demonstrate the outcomes of data science models to stakeholders, creating non-misleading visualizations is a formidable challenge. To empower data scientists in this task, we propose a set of interventions designed to enhance clarity, accuracy, and readability. At the beginning of the visual data analytic project, interventions can be designed to provide guidance on selecting appropriate visualization types based on the nature of the data and the insights to be conveyed. For example, when dealing with time-series data, data scientists can receive hints that recommend line charts for trend analysis or heatmaps for pattern recognition. Apart from the visualization types, interventions could encourage data scientists to thoroughly consider what color encoding to use in the visualization. For instance, interventions can function as a pop-up suggestion offering predefined color palettes optimized for different types of data visualizations, such as categorical, sequential, or diverging data. These palettes take into account factors like colorblind accessibility and perceptual uniformity, helping data scientists select colors that are easily distinguishable and interpretable by a broad audience. Interventions can also suggest the use of color with purpose, such as recommending using specific colors to highlight certain data points or emphasize trends if the visualization is detected and considered to be lack focus. To mitigate the risk of unintentional misrepresentation, interventions can incorporate algorithms that analyze visualizations for potential misleading patterns. If a visualization inadvertently emphasizes a misleading trend, such as distorted scales or truncated axes, data scientists can receive alerts and suggestions for correction. After a visualization is implemented, interventions can nudge data scientists to proactively ask for feedback from stakeholders or end-users so they can iterate on the visualization design for potential improvement. 
\leilani{The only responsible intervention here seems to be suggesting colorblind friendly color palettes, which I would argue is a technical solution that does not require the user.}





% \subsection{Exploring Diverse Intervention Design Possibilities}




==> sections/abstract.tex <==
% Data science pipelines influence many of our daily decisions, from what we buy to who we work for and even where we live. When designed incorrectly, these pipelines can easily propagate social inequity and harm. Traditional solutions to these problems emphasize \emph{technical satisfaction} via mitigating biased data and algorithms.
% In this paper, we explore opportunities to redefine responsible data science to encompass not only technical satisfaction but also behavioral responsibility, i.e., the patterns of behavior exhibited by data scientists that may lead to positive or negative social outcomes
% we explore a complementary opportunity to elevate \textit{ethical rigor}, i.e., to help the analysts who use data science tools to change potentially harmful or irresponsible 
% \emph{behaviors} that can contribute to downstream injustices and inequities. 
% \emily{todo: discuss "ethical" v. "responsible" terminology}
% We review existing knowledge of data science workflows, ethics guidelines from AI/visualization 
% % \emily{this bit may shift if we find a different ethical framework}, 
% and behavior change models and techniques from cognitive and clinical psychology. 
% We synthesize a definition of responsible behaviors we want to promote in data science practices. We review existing theories from cognitive and clinical psychology that encourage behavior change interventions in the context of data science. We integrate this knowledge
%for navigating the space of possible \emph{behavior change interventions} that could be implemented within data science tools.
%In this paper, we introduce a theoretical framework for implementing \emph{behavior change interventions} directly within data science tools.
%This framework integrates existing knowledge of data science workflows with behavior change models from cognitive and clinical psychology.
% to envision in situ interventions for encouraging behavior change towards responsible data science. We present several examples of interventions that could be implemented to interrupt and redirect potentially negligent practices while reinforcing responsible behaviors, and conclude with a call to action to our community to explore this new research area of behavior change interventions for responsible data science.

    
Data science pipelines inform and influence many daily decisions, from what we buy to who we work for and even where we live. When designed incorrectly, these pipelines can easily propagate social inequity and harm. Traditional solutions are technical in nature; e.g., mitigating biased algorithms. In this vision paper, we introduce a novel lens for promoting responsible data science using theories of behavior change that emphasize not only technical solutions but also the behavioral responsibility of practitioners. By integrating behavior change theories from cognitive psychology with data science workflow knowledge and ethics guidelines, we present a new perspective on responsible data science. We present example data science interventions in machine learning and visual data analysis, contextualized in behavior change theories that could be implemented to interrupt and redirect potentially suboptimal or negligent practices while reinforcing ethically conscious behaviors. We conclude with a call to action to our community to explore this new research area of behavior change interventions for responsible data science.


==> sections/brainstorm.tex <==
\section{Reference List}
Hereby we list the papers and their summaries for why they are useful for further writing reference.
\subsection{Behaviour change models}
\begin{itemize}
    \item \textbf{Digital Behaviour Change Interventions to Break and Form Habits}\cite{Pinder2018DigitalBC} surveyed a number of psychological behaviour change(BC) model and proposed a BC model to break and change habits in digital context. We could use it's survey part(section 2: THEORIES OF BEHAVIOUR CHANGE) to see their comparison of different BC models.
    \item \textbf{The Behaviour Change Wheel: a new method for characterising and designing behaviour change interventions}\cite{michie2011behaviour} proposed a BC model: COM-B model and associated interventions/policies that interplay to influence the BC process. This model will be our main model for transplanting to DS domain.
   
\end{itemize}

\subsection{Machine Learning Pipeline}
\begin{itemize}
    \item \textbf{Passing the Data Baton : A Retrospective Analysis on Data Science Work and Workers}\cite{crisan2020passing} proposed a DS pipeline which we could adapt to use as the backbone DS pipeline we refer to for designing BC model in DS.
    \item \textbf{Human-AI Collaboration in Data Science: Exploring Data Scientists’ Perceptions of Automated AI}\cite{dakuo} proposed a workflow for DS in its figure 1: Typical steps of a data science workflow, consisting of three high-level phases: data preparation, model building, and model deployment. It could be referred as our DS pipeline as well.
    \item \textbf{How AI Developers Overcome Communication Challenges in a Multidisciplinary Team: A Case Study}\cite{AIdev} proposed a working pipeline in DS in which different roles of DS in AI team and stakeholder team are specified: An AI team consults and implements AI solutions. It normally consists of technical and business representatives. A Stakeholder team requests help from a AI implementation team. They are knowledgeable in their domain, however lack knowledge in ML or AI. In this architecture the job preference of DS roles in two different teams are distinguished. 
\end{itemize}



\subsection{Factors in Data Science/Machine Learning}

\begin{itemize}
    \item \textbf{Defining an Analysis: A Study of Client-Facing Data Scientists}(Remco Chang, Tufts)\cite{10.2312:evs.20191173} categorizes the need of data scientists into three classes according to the level of clarity with which clients are able to express their analysis needs to data scientists, authors further propose three types of solution tactics that how data scientists can help with clients with different clarity: High Clarity Needs: Working Backwards; Medium Clarity Needs: Probing;  Low Clarity Needs: Recommending.
    
    \item \textbf{How Data Science Workers Work with Data: Discovery, Capture, Curation, Design, Creation}\cite{howdsworks} set five approaches to data along a dimension of interventions: Data as given; as captured; as curated; as designed; and as created. Authors listed Human interventions in data science work practices in figure 1, which could be useful to refer to potentially. \emily{may give some ideas for framing our interventions, but doesn't strike me as particularly relevant for our contextual factors}
    
    \item \textbf{Human-AI Collaboration in Data Science: Exploring Data Scientists' Perceptions of Automated AI}\cite{dakuo} interviewed 20 data scientists to ask their view on how DS's perception of AutoAI,in its 5.1.1-3, it elaborates the definition of DS as a role in business, challenges of industrial data scientists, and collaborative practices in real life DS projects. These contents can be referred to in our work.
    
    \item \textbf{How do Data Science Workers Collaborate? Roles, Workflows, and Tools}\cite{amy} presents the result of a large scale survey to data scientists(184 participants) on (1) role-based analyses of collaborations in DS. (2) how collaborations are done in different stages of data science projects(see its Figure 5). (3) an analysis of collaborative tools usage across the stages of data science projects(see its Table 2).
    
    \item \textbf{How AI Developers Overcome Communication Challenges in a Multidisciplinary Team: A Case Study}\cite{AIdev} presented a case study on how AI developers overcome communication challenges across roles in the AI development lifecycle. It report on the types of communication gaps that AI developers face, how AI developers communicate across disciplinary and organizational boundaries, and how they simultaneously manage issues regarding trust and expectations.
    
    \item \textbf{Human Factors in Model Interpretability: Industry Practices, Challenges, and Needs}\cite{humanfac} described roles, processes, goals, and strategies around interpretability practiced by ML practitioners. Interpretability plays a vital role in data science working pipeline, we could cite this work when talking about interpretability in feature engineering and model results. 
    
    \item \textbf{Factors Influencing Effective Use of Big Data: A Research Framework}\cite{frame} identified 41 factors that influence the effectiveness of big data projects and further clustered these factors into 7 themes, namely data quality; data privacy and security and governance; perceived organizational benefit; process management; people aspects; organizational aspects; and systems, tools, and technologies. This work can serve as a guideline for contexual factors in DS. \emily{this sounds the most relevant to me, particularly management, people, and organizational aspects}
    
    
    \item \textbf{Big data team process methodologies: A literature review and the identification of key factors for a project's success}\cite{Saltz2016BigDT} summarized the success factors in big data projects into 5 dimensions: data, governance, process, objectives, team, tools.(see its TABLE 5. Success factors for Big Data Projects) \emily{teams may be useful here}
    
    \item \textbf{Towards A Process View on Critical Success Factors in Big Data Analytic Projects}\cite{Gao2015TowardsAP} analysed the success factors in big data projects and grouped them into three categories: people, process and technology(See its table 2 for details). \emily{people part seems relevant, but perhaps narrower scope} 


\end{itemize}

Among all literature related to factors in DS/ML, in order to systematically review the contextual factors in DS that lead to behaviour change, i believe \cite{frame}\cite{Saltz2016BigDT}\cite{Gao2015TowardsAP}did a great job on listing and categorizing factors that influence DS success though their focuses are slightly different.\cite{frame} was published on Information & Management journal on 2020 with 94 citations; \cite{Saltz2016BigDT} was published on  International Conference on Big Data on 2016 with 94 citations; and \cite{Gao2015TowardsAP} was published on Americas Conference on Information Systems on 2015 with 90 citations(all citations data is provided by Google Scholar). I personally think \cite{frame} and \cite{Saltz2016BigDT} are more related to our topic and more systematic comparing to \cite{Gao2015TowardsAP}.





When doing literature search for factors that influence behaviour changes in data science and machine learning,  i found there are a wide variety of roles within data science, ranging from the scientists and engineers who collect and clean data and train and deploy models to leaders
and executives who define policies around data governance and ensure use of data conforms to government regulations. Thus i imagine such question can be evaluated in different context: \textbf{(1)} It could be considered in a rather simple and technical context: dataset is as given, and major work of data scientists focus on dealing with data processing + model building. \textbf{(2)} In the second context, data needs to be collected by data scientists before they run models to analysis it. In such context, factors need to be considered both in terms of data quality and data sense making(domain knowledge). In some cases even the ground-truth(labels) are not obvious\cite{howdsworks}. \textbf{(3)} In tech companies, the job content data scientists should do are clear and concrete: given some data + project context + goal, analysis and optimize towards some target functions. While in some traditional industries or business divisions, data scientist is a broad job title and job descriptions can be very different. Given  the level of clarity with which clients are able to express their analysis needs to data scientists\cite{10.2312:evs.20191173}, client-facing data scientists need to help clients to clarify the problem they face, what goal they want to achieve eventually and further formalize their business analysis pipeline before actually collect and analysis their data. Such role requires expertise in both technical skills and consulting skills. My opinion here is: we should decide if we want to be precise and focus on one or two contexts in our paper, or we want to discuss each context and potentially include all possible contexts.
\emily{I agree with your assessment of the papers you found. I lean towards using one of these frameworks that covers broad categories so that (1) we can cite it and (2) are exhaustive in some sense. But then we can identify several examples within those categories that are more specific. For the sake of whatever table we might build though, it will be nice to have a pre-defined scope of categories, even if they are broad}

\leilani{A limitation of \cite{frame,Saltz2016BigDT} is that they are more from a company perspective than a societal/cultural perspective. As a result, they do not touch on cultural issues in data science such as data privilege or data justice. We augment the ``contextual factors'' dimension to also incorporate broader societal influences on data science practice, which we delineate using ``industrial'' and ``societal'' context subcategories.}

\leilani{Potential next steps: What papers are trying to measure any interventions with respect to behavior change? Are people implementing behavior change interventions in data science? How might metrics from behavior change for digital health map to data science?}

\subsection{Factors in Psychology that influence Performance/Productivity}

\begin{itemize}
    \item Some Social Factors Related to Performance in a Research Organization\cite{10.2307/2390926} found the level of individuals' scientific performance is found to be higher under the following conditions:(1)Strong personal emphasis placed upon science-oriented values of using one's abilities, having freedom to pursue original ideas, and making contributions to basic scientific knowledge; (2) Frequent (daily) contact with several scientific colleagues who on the average have been employed in settings different from one's own, who stress values different from one's own, and who tend to work in scientific fields different from one's own; (3) At the same time, frequent contact with at least one important colleague who has similar professional values; (4) A chief and a major colleague one of whom is in the same scientific discipline and the other in a different one, rather than both similar or both dissimilar; (5) A chief who gives neither complete autonomy nor excessive direction, but who frequently interacts with subordinates and who also gives them the opportunity to make their own decisions.  \textbf{In addition to these findings on scientific performance, analyses of scientists' motivations and attitudes in twenty laboratories show that:} (6) Motivation and sense of progress toward scientific goals are stronger under laboratory chiefs who themselves are highly competent and motivated individuals; (7) Motivations and attitudes also tend to be stronger under laboratory chiefs who employ participatory rather than directive or laissez-faire leadership
\end{itemize}

\section{Reasoning for Choosing components in Behaviour Change Model}

The structure of behaviour change for data science are mainly borrowed from Fogg behaviour model\cite{fogg} and \cite{michie2011behaviour}, while-as we also believe the efficiency and success of data science/machine learning are also influenced by contextual factors which is some factors data scientists are subject to as an individual. These contextual factors are  borrowed from \cite{frame} and \cite{Saltz2016BigDT}, and are further categorized into industrial and societal factors.

\subsection{Capability}
The capability of behaviour change model in data science is borrowed from \cite{fogg}, Fogg behaviour model consider an individual's capability of encouraging a behaviour consists of six factors: time, money, physical effort, brain cycles, social deviance and non-routine, which can be adapted from a general psychological concepts into concrete meanings in data science scenarios. We transplant time factor into Time Limit/Deadline in data science, meaning the amount of time that can commit to the project, or the time amount given some certain dead lines. We borrow the money factor and interpret it as Computational Resource in data science, meaning the computational resources the ML practioner can access, e.g. GPU,CPU, number of threads, remote cluster access. We interpret it as the amount of energy, effort and vigour that ML practioners input to finish the project. Brain cycles can be illustrated as the mental readiness for ML practioners to successfully start, execute and finish a project, including the knowledge-set, mindset, know-how, blueprint of specific plans and confidence. Social Deviance can be understood as ML practioners' awareness of if the  target behaviour are considered proper and acceptable to other peers and collaborators given the coding context. And Non-routine can be understood as People tend to find behaviour simple if they are routine behaviours, thus deciding to do certain other behaviours demands ML practioners to have the ability of stepping out of some comfort zone.


\subsection{Motivation}
Motivation sub-category indicates the factors which generates self-motivation in the process of encouraging behaviour. In the COM-B model\cite{michie2011behaviour}, motivation consists of reflective thought and automatic response, while Fogg behaviour model believes motivation consists of pleasure/pain, hope/fear and social acceptance/rejection. In data science scenarios, we believe reflective thought and automatic response are fundamental factors that inter-plays to encourage behaviours, while pleasure/pain and hope/fear are also motivators that stimulates the occurrence of behaviours. We summarize the pleasure/pain and hope/fear in Fogg behaviour model as anticipation in behaviour change model in data science. Anticipation includes fear and hope -- fear of not finishing the project, getting bad result or miss the deadline; hope for something good happen(turn in the project in time, getting good result, gain personal growth via doing this project). Reflective thought can be interpreted as follow: given certain feedback, ML practioners need to examine what's the choice for next move. For example, if the model performance is poor, what is the most likely part to be responsible for that? Was it data, processing methods, parameter, model,pooling method? Automatic response
 stands for how habits, emotional responses and impulses might automatically direct our behaviour, almost without thinking. For example how to preprocess a sparse dataset before applying K-NN for clustering.
 
\subsection{Opportunity}
Opportunity sub-category is borrowed from Fogg behaviour model. Spark and Facilitator encourages behaviours when actor has different motivation and capability, signal opportunity helps to associate and remind the occurrence of a behaviour. Spark opportunity helps when we have capability but low on motivation. It could be some interior willing to warn ourselves and fight against procrastination when a dead line comes. Or some GitHub logs from collaborators showing that they made some progress and are waiting for updates from your part. Facilitator opportunities help behaviour change when we have motivation but low on capability. It could be some python plot library that make drawing figures easily, or some existing packages that simplifies our input for implementation. Signal opportunities serve as reminders to perform the target behaviour. The signal opportunity doesn't change motivation or capability, it just serve as a signal to indicate when is appropriate to do something. For example the debugger tool in VS Code provide you an opportunity to know where goes wrong in your code.

\subsection{Contextual Factors}
Other than the interior factors, there are some environmental and exterior factors that could also influence behaviours. These exterior factors could come both from industrial and societal. Industrial includes realistic concrete factors that directly influence the process of taking action, while societal factors represent some organizational elements that may not influence behaviours directly, but influence the mental process and decision-making. The factors we present here are collected, simplified and re-organized(synonyms are combined) from \cite{frame} and \cite{Saltz2016BigDT}.Some factors in Team and People category are extended and augmented from the factors proposed in these two papers.

\\
\textbf{\textcolor{red}{Contents above this line are for brainstorming and notes taking for the useful papers we found, and will be deleted in the formal writing}}

==> sections/old_3.bcds_not_used.tex <==
\section{A Framework for Behavior Change in Data Science (BCDS)}
\label{sec:bcds}


\ziwei{
In this section, we basically only use TDF as a theory framework, and adopt it into data science area. Explain why DS need this frame, and why we pick TDF as a basic to extend to DS. Need to remove COM-B in this section.
}

% \begin{comment}
% \ziwei{\textbf{Subsection Motif:} In this section we introduce how we examine the relationship between capability, motivation , trigger and contextual factors. And then we discuss: given such relationship, how we scope the interactions between these 4 factors with the high-level data science pipeline \autoref{fig:teaser}.\\

% \noindent \textbf{Breakdown Contents}: (1) Introduce the how we scope the relationship between capability, motivation , trigger and contextual factors. Discuss motivation + capability are independently influenced by contextual factors(see Miro meeting notes for September 15th). (2) Given the relationship between capability, motivation, trigger contextual factors and interventions, discuss how these 5 elements participates in the data science workflow, and illustrate the diagram(teaser fig) here. (3) Discuss the down-stream effect of intervention could have for the end result of a data science project.}
% \end{comment}

% Contextual factors independently influence(increase/decrease) motivation and capability of making a certain behavior, it sort of like the environment that surrounds a person, like air, like oxygen.

% Opportunity(where we could apply interventions before the decision of a certain behavior is made) functions like a amplifier/decreaser, which is the last chance we could input to encourage/suspend the occurrence of a behavior. It independently influences capability and motivation, and the sum of the amplified/descreased capability and motivation put together decides the occurrence of a behavior.

% The therefore resulted behavior independently influence each stage of ML pipeline.Each stage have different settings for capability, motivation, opportunity and contextual factors; and the result of previous stage(s) may influence the contexual factors, capability, motivation of the current stage. Thus, one special and vital character for designing behavior change interventions in Data Science is we should consider such process is cascaded, continuous; the interventions we design could have down-stream effects at the end result of a ML model. This is how behavior change Interventions in data science are unique and why studying such problem is important as well.

 % \ziwei{Adjusted according to our discussion between me and Ameya. }
 
%Having described the data science pipeline (\autoref{sec:ds_pipeline}), the desired ethical behaviors (\autoref{sec:ethical_behaviors}), and the theory behind behavior change (\autoref{sec:bc_psych}), 
Having described the critical factors for ethical data science in~\autoref{sec:background_ds}, we now tie it all together to describe our proposed framework for Behavior Change in Data Science (BCDS).
We first define the terminologies we use in this framework, and then describe the interaction between them. We use the word `agent' to represent the data analyst, and the word `action' to represent one or more steps of the data analysis process. %, in our descriptions of the terms.


\subsection{Components of the Framework}
\label{sec:components}
%\emily{Let's add operational definitions here: really precisely describe in one sentence each, what we mean by capability, motivation, opportunity, trigger, intervention, behavior, etc. Maybe in a table? Three columns: term, definition, example}
%\emily{in the writing make it clear how these terms differ from the way they were originally used}
We begin by first operationally defining the concepts that comprise BCDS. We adopt some terms directly as they are used in COM-B~\cite{michie2011behaviour} and in TDF~\cite{atkins2017guide}, and slightly alter others to more closely match our data science focus. \autoref{fig:teaser} shows the components of our framework. %Since we do not have a good behavior change model for data science context, we draw inspiration from behavior change work in psychology and its applications in medical practices. We avoid devising new terms for behavior change in the data science context without the required scientific rigor, and rely more on the simple yet comprehensive COM-B model as also referred to by the TDF model. We recognise the need to create a detailed behavior change framework tailored for data science as future work, and present our current work as a vision paper towards the tangible use of such a framework.
We mark such modified/new terms with an asterisk to separate them from those directly borrowed from prior work.

%\begin{itemize}[noitemsep]
%\item 
\medskip
\noindent\textbf{Instruments of Behavior Change} %\emily{mark w/ asterisk?} 
%include constituent terms and their operational definitions for 
describe \textit{how} we bring about the desired behavior change in data science.
\begin{itemize}
    \item \textbf{Interventions} are triggers, as defined in FBM~\cite{fogg}, %\emily{I thought action was performed BY the agent, not ON the agent? is there another word we can use here so that it's not potentially confusing?} 
    imposed on the agent, to bolster the level of their \fbc{capability}, \fbc{opportunity}, or \fbc{motivation}, thereby affecting their behavior. In other words, interventions are instances of the BCT described in~\autoref{sec:bc_psych}. In data science, a few examples could include \bct{training the agent} on math/statistics background (increases \fbc{capability/motivation} to analyse data correctly) or showing the agent which part of the data they have focused on thus far in a data analysis session, to encourage them to account for and balance their data exploration~\cite{wall2017warning,wall2021left} (increases \fbc{capability/opportunity}).
    
    \item \textbf{Disruptors*} are catalysts or %\emily{may want to avoid using signal, since that's one of the types of interventions/triggers we discuss later}
    events that indicate when to introduce an appropriate intervention. We adopt this terminology from the Fogg Behavior Model~\cite{fogg} to capture the conditions by which an intervention may be triggered. In data science, a possible disruptor could be when an analyst switches to a new phase of the data science pipeline, \eg switching from \dsp{analysis} to \dsp{deployment}, an intervention could be introduced to remind the analyst to check if the model tries to infer for populations which were missing in the training data.
    % to facilitate positive behaviors towards more ethical data science practice.
    %While the Fogg model uses the term ``trigger,'' it more closely relates to our concept of Intervention (above). 
    If the intervention is the \textit{how}, we use the term disruptor to describe the \textit{when}. 
    
    \item \textbf{Behaviors*}, in our framework, are practices related to data science. Behaviors can involve actions that lead to more ethically rigorous processes, such as performing fairness checks on data or ensuring data privacy; or on the contrary, behaviors could also potentially lead to ethically irresponsible processes, such as neglecting the unbalanced  distribution of socially sensitive features in a dataset, or unreasonable train-test split of a dataset. 
\end{itemize}

\medskip
%\item 
\noindent\textbf{Contextual Factors*} represent the sum total of the agent's internal state and external circumstances. %, which drive their actions
It is the superset of the analyst's \fbc{capabilities}, \fbc{opportunities} and \fbc{motivation}, as defined by the COM-B model, and the stage of the data science process that the analyst is in. We propose this term to identify the complete context in which the agent operates, which is critical to executing successful behavior change interventions~\cite{michie2005making} and data science projects~\cite{al2020critical,Saltz2016BigDT,Sejahtera2019factors}. 
% \ziwei{Right now contextual factors sound like a mixture of internal + external factors instead of the sum of industrial and social factors. In such case, it makes sense to put data quality/infrastructure in opportunity.

\begin{itemize}
    % \item \textbf{Contextual factors} are part of an individual's circumstance and experiences surrounding and implicitly influencing their data science practice. Contextual factors include \textit{industrial factors} relating to data quality, data privacy, and systems; and \textit{societal factors} including team dynamics, process management, and organizational factors, shown in \autoref{fig:context}. These terms are defined in supplemental materials.

    \item \textbf{\fbc{Capability}}, as defined by the COM-B model, is \definition{the individual's psychological and physical capacity to engage in the activity concerned.} This factor is internal to the agent performing the action. In the data science context, \fbc{capability} is more about mental than physical traits, and it includes factors like \fbc{knowledge} and \fbc{skills} relevant to data analysis or the data domain, \fbc{memory}, \fbc{attention} and \fbc{behavioral regulation skills} of the analyst (\autoref{fig:com-b}).

    \item \textbf{\fbc{Opportunity}} is defined as \definition{all the factors that lie outside the individual that make the behaviour possible or prompt it} and is a factor external to the agent performing the action. In other words, the right \fbc{opportunity} enables an analyst to make the desired change in their behavior, whereas the wrong \fbc{opportunity} or lack of it hinders the analyst's \fbc{capability} or \fbc{motivation} to change. Importantly, this captures many otherwise implicit aspects of data science practice, including an individual's context of work and privilege. The social, physical and digital environment in which the agent functions, has a significant influence on their behavior~\cite{skinner,michie2005making,Neal2006HabitsARP,wood2016psychology,pinder2018digital,bandura2001social}. These environmental factors affect behavior by providing some kind of \fbc{opportunity} to the agent, as categorised by the TDF domains of \fbc{Social influences} and \fbc{Environmental Context \& Resources}~\cite{cane2012validation}. In the data science context, it contains \fbc{industrial factors} relating to data quality, data privacy, data privilege, and data justice, and \fbc{societal factors} including team dynamics, process management, and organizational factors. \autoref{fig:com-b} and \autoref{sec:ds_pipeline} (under \textit{success factors for data science projects}) provide more examples on such environmental factors. 
    %\emily{does it?}

    \item \textbf{\fbc{Motivation}} is defined as \definition{all those brain processes that \textit{energize} and direct behavior.} This factor is internal to the agent performing the action. It can be further categorized into \textit{automatic motivation} which includes factors like \fbc{emotion} and \fbc{reinforcement}, and \textit{reflective motivation} which includes factors like \fbc{optimism}, \fbc{intentions} and \fbc{beliefs}, as shown in \autoref{fig:com-b}. Motivation essentially relates to an analyst's willingness to perform a target behavior.

    \item \textbf{\dsp{Data Science Pipeline Stage}*} represents the data science context that the analyst functions in. 
    %In~\autoref{sec:ds_pipeline}, we describe the data science pipeline formalism (also shown in~\autoref{fig:teaser}) which identifies 4 high-level stages. 
    The analyst functioning in any of these stages or transitioning between stages, forms an important input to our framework to decide when to intervene (\textit{disruptor}) and how to intervene (\textit{intervention}).
\end{itemize}

%We refer to Fogg model to define the capability in data science practices. 
%The Fogg model describes that this concept further consists of \textit{time, money, physical efforts, brain cycles, social deviance, and non-routine}. \emily{potentially move this to the section on behavior change, and only describe our adoption of the term here?}
% In the data science context, we posit that capability includes \textit{time limit/deadline, computational power, physical efforts, brain cycles, social deviance, non-routine}, depicted in \autoref{fig:cap}. 
%\emily{I want to read through our descriptions of these -- having a hard time remembering what we discussed}
% The detailed definitions of these components are provided in the supplementary materials. 
%file\ziwei{add autoref to additional file here}.

% \emily{is Opportunity in TDF?} \ameya{not explicitly, but TDF domains have been mapped to Opportunity in~\cite{cane2012validation}}
% moved this above Motivation just for consistency with Acronym}\ziwei{TDF has two versions, neither of them includes opportunity. Also i sense that good data/infrastructure should belongs to industrial factors, which is a part of contextual factors. RE Emily's comment: i also lean towards removing fig 2.}
% Thus, opportunity depends on an analyst's capability and motivation, which can be modulated by appropriate interventions.

%\emily{not sure this is particularly useful to see in the figure given its description here -- candidate to remove fig. 2? }

%\end{itemize}

\subsection{Component Interactions}
The components described in \autoref{sec:components} influence one another in nuanced ways. In this section, we describe how they interact with one another specifically in the data science context. \autoref{fig:teaser} also shows these interactions.
%\emily{Grouping together Capability and Motivation in one section seems good cause both models include that.}
%\emily{a separate subsection on Contextual Factors might be nice}\ziwei{I group them together because they are all in the blue box in the teaser figure and they interact with each other before interventions play a role in the occurrence of behaviors. Group them together could make it easier to introduce the interaction between these three things.}
%\emily{A subsection that groups together Trigger and Opportunity might also be nice}\ziwei{this comment will be addressed after we have a mutual agreement on distinction between intervention, trigger and opportunity.}
%\emily{a subsection on Interventions and Behaviors could also be good?} 
%factors of  behavior change in data science, the next step was to link the components of behavior change in data science model with the data science pipeline. In this section, we introduce a new behavior change intervention model in data science: 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1.1 \textwidth]{figs/4_factors.pdf}
%     \caption{The 4 factors that accounts for the occurrence of behavior in data science. \emily{can we update this figure to annotate which model these components come from? and potentially add labels to some of the edges for instances where it is not a subset relationship}}
%     % \caption{\ziwei{One cluster can have multiple rule lists, the order of rule lists describe how well each rule list reflects strategies within the cluster are different from those outside in a descending order.}}
%     % TODO: trim from sides to adjust for white space
%     \label{fig:framework}
% \end{figure}


\begin{figure}
  \includegraphics[width=0.9\linewidth, trim={0 0 18mm 0}, clip]{figs/com-b_ds.pdf}
  % TODO: trim from above and below to adjust for white space
  \caption{Zooming in on contextual factors of the COM-B model~\cite{michie2011behaviour} relevant to BCDS.}
  \description{}
  \label{fig:com-b}
\end{figure}



% \subsubsection{Capability, Motivation and Contextual Factors}

\subsubsection{\fbc{Capability, Opportunity, \& Motivation}}

% Within the red box in \autoref{fig:teaser}, \textit{capability}, \textit{motivation}, and \textit{contextual factors} represent internal and external characteristics of an individual that collectively influence the \textit{opportunity} for a behavior to occur. However, these factors interact with each other in nuanced ways.

The components of the COM-B model collectively play a part in influencing the behavior of the agent. These factors also interact with each other in nuanced ways as described in~\cite{michie2011behaviour}. %in~\autoref{fig:com-b}.
% Given that capability and motivation are the very fundamental factors that nudge the occurrence of behavior, understanding the interplay between these two factors becomes a starting point of BCDS. 
Understanding this interplay becomes a starting point of BCDS.
In data science, \fbc{capability} can influence the magnitude of an agent's \fbc{motivation} to perform the target behavior. 
For example, diminished \fbc{capability} of remembering different kinds of statistical tests for different purposes, can affect the \fbc{motivation} to apply the appropriate test for the task at hand. %Conversely, given abundant motivation to execute a data science practice, an individual's capability can be reinforced and boosted in the long run if they continue to practice that behavior e.g., learn-by-doing practice on PyTorch following some ethically-aware tutorials can quickly familiarise a beginner and boost capability on coding ethically rigorous deep learning models.
Similarly, \fbc{opportunity} can also influence the agent's \fbc{motivation}. For example, availability of a streamlined tool to organise data and track the proportion of samples for different classes for a classification task can make the analyst more confident about the correctness of their workflow, thereby increasing their \fbc{motivation} to practice ethical ML.

% \ameya{TBD: Cite theories of behavior change for the speculation on slow vs fast changes or short-term vs long-term habit changes}
Influences of \fbc{motivation} (psychological state internal to the agent) on \fbc{capability} (psychological/physical state internal to the agent) and \fbc{opportunity} (external to the agent) are usually indirect and happen in the long-run~\cite{michie2011behaviour, willmott2021capability}, and are thus not directly relevant for our BCDS framework. %\emily{does internal = psychological and external = physical?} \ameya{not exactly, internal means internal to the agent, so both physical and psychological are internal factors}
For example, the data analyst's \fbc{motivation} to improve the analysis workflow at his company through the use of better tools (\fbc{opportunity}) might require communicating these changes to the higher-ups. Such a change can take considerable time and subtlety in navigating organizational culture. As another example, the analyst's \fbc{motivation} to learn new types of deep learning models can improve \fbc{capability} in terms of knowledge, but this kind of learning can take multiple days or weeks.% \emily{italicizing the model components might improve the comprehension of these statements as they relate to our model; i.e., italicize motivation, capability, etc. throughout this explanation}

BCDS focuses on in-the-moment interventions for short-term behavior change, \ie we focus on influencing behavior by increasing \fbc{motivation} and \fbc{capability} of the analyst to perform ethical data analysis. We describe some examples of such interventions in~\autoref{sec:interventions}. Influencing data science behavior by increasing \fbc{opportunity} is not in-the-moment, since it entails changing the external environment of the analyst, which takes significant time and subtlety. It is also difficult to do via purely software interventions, and hence is out of scope for our framework.% Since we only consider software interventions in data science workflows, influencing \fbc{opportunity}---external environment of the analyst, through software interventions is out of scope for our framework.

% While capability and motivation are internal characteristics of an individual, they are nonetheless influenced by changes to the opportunity~\cite{skinner}.

% Contextual factors independently reduce or amplify motivation and capability of executing a certain behavior.

% For example, if the performance management of the organization is not properly defined, this can weaken data scientists' motivation by providing incorrect incentivization. Another example is education, in terms of skills and knowledge in data science, the capability of an analyst who received a degree in a computing-related discipline such as computer science may be higher than an individual who is self-taught in data science. 

% Other characteristics of an individual's experience in the world, including their privilege, can heavily impact both capability and motivation, and vice versa. An individual with high motivation can overcome deficits in capability or privilege.
%Similarly, it is objectively challenging to train a successful model from a low quality dataset. 
%This context may result in a data scientist's diminished capability and may simultaneously weaken one's motivation. 
%Capability, motivation, and contextual factors collectively determine the intrinsic status(shown in the blue dashed box of \autoref{fig:teaser}), and such status could be further intervened by long-term or short-term behavior change interventions.




% \subsubsection{Disruptors, Interventions, and the Data Science Pipeline}
\subsubsection{Disruptors, Interventions, and the Contextual Factors}
%Given the right opportunity (as characterized by an an individual's context, capability, and motivation), we may \textit{disrupt} an analyst's data science practice with an \textit{intervention}. 

Given a certain state of the contextual factors of the analyst as characterized by the \fbc{capabilities}, \fbc{opportunities}, and \fbc{motivations} available, and the stage of analysis the analyst is in, we may interrupt the analyst's action with an \textit{intervention}, when we detect a \textit{disruptor}. 
Both the disruptor and the intervention itself, are inferred from the contextual factors. For instance, a disruptor may be based on the transition between phases in the data science pipeline, or it may be based on a specific sequence of analysis actions, giving hints about the technical knowledge (\fbc{capability}) of the analyst~\cite{wall2017warning}.
Furthermore, the interventions we envision will be informed by triangulating an agent's position in space of \fbc{capability}, \fbc{opportunity}, and \fbc{motivation}, and may likewise be injected into or embedded in the data science pipeline, \eg as computational notebook extensions.
% Hence in \autoref{fig:teaser}, we depict these components with a common color, green. Commenting this out, since it implies we also show contextual factors in green, which we don't. Anyway, this may interfere with the color code chose for BCT (disruptor and intervention instances)
%Based on the interplay of capability, motivation and the certain given contextual factors, we establish opportunity as the generated posterior time window to nudge the desired behavior. Such intrinsic generated opportunity is the last chance we could pitch in and increase/decrease the possibility of the occurrence of desired behavior, and a properly designed intervention can significantly facilitate the occurrence of the desired data science practices. 
%To that end, the design of the intervention should suit both (1) the characteristic of the application scenario(current data science phase), and (2) the expected timing that the intervention would eventually work out(when). 
% (if the intervention designed to function as an in-the-moment trigger to help with short-term behavior change, or it creates a long-term opportunity that accounts to a habit formation).
% To that end, we formalize disruptor as the catalysts that signify when to introduce an appropriate intervention. 
%Therefore, we combine these two needs and formalize them as disruptor: a catalyst that signify when to introduce an appropriate intervention given the characteristics and nature of current data science phase. In brief, the nature of the current data science phase informs the disruptor, and given the disruptor, a appropriately designed intervention will ideally grasp the opportunity to independently promote the capability or motivation, r both, and escalate the sum of the amplified capability and motivation towards the occurrence of a desired behavior \autoref{fig:teaser}.


\subsubsection{Intervention Feedback Loop}
\label{sec:downstream}

To design context-aware behavior change interventions to promote responsible data science, one must consider the feedback loop: behaviors impact the contextual factors, \ie the characteristics of the data science pipeline as well as the agent's intrinsic qualities like \fbc{capability} and \fbc{motivation} (in the short-term), and the \fbc{opportunities} available (in the long-term).
Furthermore, it may be the case that multiple behavior change interventions are deployed. 
The cascaded design of the chained interventions in the data science pipeline could prompt down-stream effects on the end result of the data science project (see \autoref{fig:teaser}). 
For instance, the end result of the data-processing (\dsp{preparation}) stage will be the input to the model training (\dsp{analysis}) stage, which could potentially lead to changes to the \fbc{capability} (\eg \fbc{behavioral regulation}) and \fbc{motivation} (\eg \fbc{beliefs about consequences}) of the analyst, and the \fbc{opportunities} available to the analyst (\eg \fbc{environmental context}) during the model training stage. 
In consequence, designing responsible behavior change interventions for the earlier stages can anchor improved ethical rigor in the later stages, as detailed in the COM-B model~\cite{michie2011behaviour} indicated by the double-headed arrows between behavior on one hand, and \fbc{capability}, \fbc{opportunity} and \fbc{motivation} on the other hand.
% This is one unique characteristic for behavior change interventions in data science: that the process is cascaded, continuous, and particularly sensitive to down-stream effects.
This makes the data science process cascaded, continuous and particularly sensitive to down-stream effects.

%\subsection{Ethical Rigors in Data Science -TBD}






==> sections/summary.tex <==
\section{Summary for the Potential Future  Collaborator}

Hi dear potential collaborator, I'm Ziwei Dong from Emory University and I'm happy to talk to you virtually. In the past two months, I've been working with Leilani and my advisor Emily to explore how could we refer to the existing canonical psychological behavior change models, and further adapt and modify them to develop a new behavior change model whose characteristics are suited to the nature of data science/machine learning domain. This project started with such a clear \textit{motivation} but with a vague path forward.
We started from searching literature on existing behavior change models, hope we could translate them into the data science domain and develop a new model, but without knowing what else we could end up finding although we wish to go beyond just developing a model.

\subsection{What factors collaboratively influence behavior in DS?
}
To kick start the project, I did some some literature survey on the existing behavior change models in psychology. After iterating on the found models we ended up agreeing on the Fogg\cite{fogg} and COM-B \cite{michie2011behaviour} models as two test-of-time models that we could refer to. These two models (Fogg model\autoref{fig:fogg} and COM-B model\autoref{fig:comb}) both argue that a target behavior is a function of capability, motivation and opportunity (in the Fogg model the terms the author used are ability, motivation and trigger, respectively). The attractive difference between these two models is: the Fogg model is more suited to identifying in-context, instant solutions for persuasion
using in the moment triggers, whereas
COM-B is better suited to more strategic
applications around broader behavior habitual formation, focused on filling
in the gaps in people’s capability,
opportunity and motivation in the long run.Such differences lead to a need for combining these two models to develop a new model for data science  behavior change interventions, since they could be designed for both in-the-moment and in the long run.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.5 \textwidth]{figs/com-b.png}
    \caption{COM-B model consists of capability, motivation and opportunity}
        % \caption{\ziwei{One cluster can have multiple rule lists, the order of rule lists describe how well each rule list reflects strategies within the cluster are different from those outside in a descending order.}}
    \label{fig:comb}
\end{figure}




\begin{figure}[t]
    \centering
    \includegraphics[width=0.5 \textwidth]{figs/fogg.png}
    \caption{Fogg model demonstrates the occurrence of a behavior as a 2-D space formed by ability and motivation, designing different types of triggers can encourage the occurrence of a certain behavior}
        % \caption{\ziwei{One cluster can have multiple rule lists, the order of rule lists describe how well each rule list reflects strategies within the cluster are different from those outside in a descending order.}}
    \label{fig:fogg}
\end{figure}




Based on these two models, the next question we started to iterate on was: is the behavior in data science domain solely influenced by capability, motivation and opportunity? Given the chance to think about this question, we started to realize all these three factors mentioned in the Fogg model or COM-B model are all internal factors of an individual, leaving the seemingly unrelated external factors (such as work deadlines, project budgets, or even individual factors related to an individual's privilege) scoped out. Thus, our next round of literature survey focused on finding the contextual (external and environmental) factors that could drive the behavior change in data science. We ended up curating a list of papers that are related\cite{Gao2015TowardsAP}\cite{Saltz2016BigDT}\cite{frame}\cite{humanfac}\cite{AIdev}\cite{amy}\cite{10.2312:evs.20191173}\cite{dakuo}\cite{howdsworks}. We further summarized them and made an taxonomy of the contextual factors in the data science domain mainly referring primarily to \cite{Saltz2016BigDT}\cite{frame}. At this moment, we built a tree-structured factor diagram which includes all potential factors that could influence a data scientist's behavior change. The diagram is shown in \autoref{fig:framework}.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.1 \textwidth]{figs/Noname Playground.png}
    \caption{As this tree is drawn in Miro, it does not allow downloading a high resolution PDF without subscription. My apologies for the inconvenience, but please refer to \cite{url} for the clearer version of the graph.}
        % \caption{\ziwei{One cluster can have multiple rule lists, the order of rule lists describe how well each rule list reflects strategies within the cluster are different from those outside in a descending order.}}
    \label{fig:framework}
\end{figure}

\subsection{In which way does these factors interact with each other and ultimately determines the behavior?
}
Given the factors we systematically summarized and grouped, a further question we thought about is: how could capability, motivation, opportunity and contextual factors inter-play to influence the behavior in data science? The following is our answer to this question. Contextual factors independently influence (increase/decrease) motivation and capability of of an individual, sort of like the environment that surrounds a person, like air, like oxygen. Opportunity (where we could apply interventions before the decision of a certain behavior is made) functions like an amplifier/decreaser, which is the last chance we could intervene to encourage/suspend the occurrence of a behavior. These interventions take place somewhere in the context of the ML or DS pipeline. Interventions independently influence capability and motivation, and the sum of the amplified/decreased capability and motivation put together decides the occurrence of a behavior. 
%The resulting behavior can independently influence each stage of the ML pipeline. 
At each stage of the DS pipeline, an individual can have different combinations for capability, motivation, opportunity and contextual factors; and the result of previous stage(s) may influence the contextual factors, capability, motivation of the current stage. Thus, one special and vital characteristic for designing behavior change interventions in Data Science is to consider this process as cascaded, continuous; the interventions we design could have down-stream effects on the end result of a ML model. This is how behavior change Interventions in data science are unique. This workflow is shown in the teaser \autoref{fig:teaser}.

\subsection{How can we guide readers to design behavior change interventions for DS practioners?}
Along the journey in this project, Leilani asked an excellent question: given what we explored already, what advice could we give the readers for them to design their behavior change interventions? How can they benefit from such a systematically examined and built framework? Luckily, we came across a serendipitous answer to this question. In the Fogg behavior model, he proposed a theory that opportunity could be classified into three types: \textbf{Spark opportunity}, which helps when we have enough capability but are low on motivation; \textbf{Facilitator opportunity}, which helps behaviour change when we have enough motivation but are low on capability; and \textbf{Signal opportunity}, which serves as reminders to perform the target behaviour (apparently, such reminders make more sense when a person has both enough capability and motivation, and the only thing he/she needs is a reminder to make sure the behavior will happen as planned). Our answer to the question Leilani asked is: we could potentially build a 3 by 3 matrix, where it shows under different combination of the magnitude of capability and motivation (low, medium and high), the types of triggers or opportunities for intervention may be most effective. It doesn't necessarily mean a person only needs one type of trigger given his/her situation. What trigger an individual needs could be some combination of all three types -- what matters is which trigger plays a more important role in how the intervention works. Thus, we performed a systematic analysis based on the definition of the three types of triggers (opportunities), and further concluded into the matrix shown in \autoref{fig:3x3}.

The three questions in the subtitles listed above are the questions we've been working on and answering so far in this project. These are some initial findings, and are not perfectly polished. This direction is a blue ocean and we anticipate there are still many findings awaiting to be dug out. At this point, potential next-steps we could explore  \textbf{theory-wise} are:
\\

\begin{itemize}
    \item Give concrete examples of what interventions we could design for each of these combinations.
    \item Examine what down-stream effects the behavior change intervention could have for the latter steps each step in the machine learning pipeline.
    \item A more systematic survey on the areas of the three subsections introduced above.
\end{itemize}

This work is a part of a funding proposal Emily and Leilani wrote together: Promoting Responsible Data Science Through Behavior Change Interventions. PIs want to first explore on the theory-wise to see what interventions we could design to promote responsible behavior in data science, and after that, we likely want to explore \textbf{application-wise} and develop a few of these interventions as plugins e.g., in JupyterLab. These two works(one on theory and one on application) will be a series of projects where the first work can provide design principles in theory to guide the specific intervention design on data science coding environments(JupyterLab and etc.). Please feel free to connect and ask questions about this project if you feel interested. I am happy to explain more.





\begin{figure}[t]
    \centering
    \includegraphics[width=1 \textwidth]{figs/3x3.pdf}
    \caption{The 3 by 3 matrix where we give high level suggestions to reader to design interventions in different situation where target individuals have different magnitude of capability and motivation, please refer to \cite{url} for the clearer version of the graph.}
        % \caption{\ziwei{One cluster can have multiple rule lists, the order of rule lists describe how well each rule list reflects strategies within the cluster are different from those outside in a descending order.}}
    \label{fig:3x3}
\end{figure}
